Leveraging Core and Uncore Frequency Scaling for Power-Efficient Serverless Workflows

Serverless workflows have emerged in Function-as-a-Service (FaaS) platforms to represent the operational structure of traditional applications. With latency propagation effects becoming increasingly prominent, step-wise resource tuning is required to address Service-Level-Objectives (SLOs). Modern processors' allowance for fine-grained Dynamic Voltage and Frequency Scaling (DVFS), coupled with serverless workflows' intermittent nature, presents a unique opportunity to reduce power while meeting SLOs. We introduce $\Omega$kypous, an SLO-driven DVFS framework for serverless workflows. $\Omega$kypous employs a grey-box model that predicts functions' execution latency and power under different Core and Uncore frequency combinations. Based on these predictions and the timing slacks between workflow functions, $\Omega$kypous uses a closed-loop control mechanism to dynamically adjust Core and Uncore frequencies, thus minimizing power consumption without compromising predefined end-to-end latency constraints. Our evaluation on real-world traces from Azure, against state-of-the-art power management frameworks, demonstrates an average power consumption reduction of 16\%, while consistently maintaining low SLO violation rates (1.8\%), when operating under power caps.

==> tables/max_load.tex <==
% \setlength{\extrarowheight}{1.4pt} % Adjust this value to increase 


\begin{table}[b]
\caption{Performance profiles of examined functions~\cite{sebs}. \recheck{mhpws na mpei kai average? isws na fugei kiolas}}
\label{tab:performance-profiles}
\centering
\begin{tabular}{c|c|c|}
\Xcline{2-3}{3\arrayrulewidth}
\textbf{}  & \begin{tabular}[c]{@{}c@{}}\textbf{max load}  \textit{(RPS)}\end{tabular} & \begin{tabular}[c]{@{}c@{}}\textbf{Latency}  \textit{(p$95^{th}$)}\end{tabular} \\
\Xcline{1-3}{3\arrayrulewidth}
\multicolumn{1}{|l|}{\texttt{\small thumbnailer}}  & 1  & 1033\\
\hline
\rowcolor[HTML]{EFEFEF}\multicolumn{1}{|l|}{\texttt{\small dynamic-html}} & 1 & 120 \\
\hline
\multicolumn{1}{|l|}{\texttt{\small dna-viz}}  & 1  & 1033\\
\hline
\rowcolor[HTML]{EFEFEF}\multicolumn{1}{|l|}{\texttt{\small compression}} & 1 & 120 \\
\hline
\multicolumn{1}{|l|}{\texttt{\small video-processing}}  & 1  & 1033\\
\hline
\rowcolor[HTML]{EFEFEF}\multicolumn{1}{|l|}{\texttt{\small img-classification}} & 1 & 120 \\
\hline
\multicolumn{1}{|l|}{\texttt{\small graph-pagerank}}  & 1  & 1033\\
\hline
\rowcolor[HTML]{EFEFEF}\multicolumn{1}{|l|}{\texttt{\small graph-mst}} & 1 & 120 \\
\hline
\multicolumn{1}{|l|}{\texttt{\small graph-bfs}}  & 1  & 1033\\
\Xcline{1-3}{3\arrayrulewidth}
\end{tabular}
\end{table}
